Indexing Cost Sensitive Prediction

Predictive models are often used for real-time decision making. However, typical machine learning techniques ignore feature evaluation cost, and focus solely on the accuracy of the machine learning models obtained utilizing all the features available. We develop algorithms and indexes to support cost-sensitive prediction, i.e., making decisions using machine learning models taking feature evaluation cost into account. Given an item and a online computation cost (i.e., time) budget, we present two approaches to return an appropriately chosen machine learning model that will run within the specified time on the given item. The first approach returns the optimal machine learning model, i.e., one with the highest accuracy, that runs within the specified time, but requires significant up-front precomputation time. The second approach returns a possibly sub- optimal machine learning model, but requires little up-front precomputation time. We study these two algorithms in detail and characterize the scenarios (using real and synthetic data) in which each performs well. Unlike prior work that focuses on a narrow domain or a specific algorithm, our techniques are very general: they apply to any cost-sensitive prediction scenario on any machine learning algorithm.

==> content/xx-data-structure.tex <==
\section{Creating the data structure}

Assumptions:

\begin{itemize}
  \item Feature $f_i$ is independent of $f_j$

  \item For each $\Delta n$ in $1 \dots N$ data points, for each $f_i$, we
  calculate the cost $t$ of running that feature on that data set. 
  
\end{itemize}

Now we can claim to be equiped with:

\begin{itemize}
\item A graph plotting input size $n$ versus expected time $t$ for each basket
of features $F \in \mathcal{F}$. We further assume we can derive, for each $F$,
a polynomial that represents this curve.
\end{itemize}

Our goal is to compute a plot like 

\begin{figure*}[h!]
\centering
\includegraphics[width=0.9\textwidth]{figures/algo.pdf}
\caption{Skyline creation}
\label{fig:tradeoff}
\end{figure*}








==> content/xx-problems.tex <==



Many machine learning models fit the basic form of accepting some structured
input $x$, computing features over that input $\mathcal F(x)$, and then
producing a prediction $y$ using some set of guiding parameters $\theta$.

$$m(\mathcal F(x); \theta) : y$$

$\mathcal F$ in this case decomposes into a set of component feature functions
$\langle f_1(x) \dots f_n(x) \rangle$. In most applications, the programmer
\textit{fixes this set of functions offline} and through relatively \textit{ad
hoc} experimental methods.  The number of features to compute in an
operationalized model can thus extend into the millions. \eob{Find citations of
some important papers which have millions of features.}

This paper explores the tradeoff between the expected \textit{cost} to compute
features $\mathcal F(x)$ and the expected \textit{error} of the model running
with those features, which we denote $error_m(\mathcal F)$. In particular,
there may be many situations in which some subset of features $F \subset
\mathcal F$ delivers a preferrable cost-to-expected-error ratio.

We call this task of selecting some $F \subseteq \mathcal F$ cost-sensitive
feature selection and denote it as a function which takes a universe of
potential features, a cost constraint, and a model input provided at runtime
and returns a list of features:

$$ select(\mathcal F, C, x) : F $$

For the first part of this paper, we consider the case where $select$ is called
once, before the model is run, and has access only to the size of the input $x$
with respect to the complexity of each feature $f_i$, which we refer to as
$c_{f_i}(x)$. For example, a feature which performed a linear scan of text
would have access to the length of text string $x$. A feature which calculated
the median of a vector would have access to the size of vector $x$. This
permits $select$ to reason about how costly each feature is to compute against
an input $x$ relative to other features.

For the second half of this paper, we relax the constraint that $F$ must be
decided before model execution and consider the case where the model may
iteratively spend its cost budget, thus computing new features with knowledge of the
results of existing features.

We defer discussion of model training to future sections.


%We consider the set of classifiers which rely on a set of features to generate
%their prediction. I.e., any one model takes the form $m(F, x) : y$ where $x$ is
%an input point, $y$ is a label (the classification), and $F$ is a set of
%feature functions and any associated metadata (such as weights) with which $m$
%makes the classification decision.

%In most machine learning applications today, \textit{the programmers fixes $F$
%offline}. For example, application-centric papers in the natural langauge
%processing or computer vision communities often contain a list of features
%used in the model presented to solve some problem. This paper consider the
%problem of dynamically selecting $F$ online in response to a cost budget.
%
%We assume the set of feature functions $F$ is drawn from a larger set of
%possible functions $\mathcal F = \{f_1, f_2, f_3 \dots f_n \}$. Each function
%$f_i$ has a corresponding cost which is a function of both the data element
%being labeled and also the data set from which this element comes $c_i(x, n)$.

%As some examples, a feature which takes an integer and returns whether it is
%positive or negative has cost $c(x, n) = 1$. A feature which takes an integer
%and returns whether it is the max integer in the dataset has cast $c(x, n) =
%|n|$. While we constrain cost to scale with respect to $x$ and $n$ for our
%investigation, our work lays foundation for more flexible cost models.  p

%\subsection{Formalization}
%
%We use the following notation through this paper.
%
%\textsc{Models.} This work considers the set of models which can be described
%
%\begin{itemize}
%  \item $m$ is a model with parameters $\theta$
%  \item $x$ is a structured object provided as input at training or test time
%  \item $\Phi$ is a collection of ``feature functions'' which transform $x$
%  into values directly usable by $m$, $\langle \phi_1(x) \dots \phi_n(x)
%  \rangle$ 
%  \item $y$ is an output of the model
%\end{itemize}
%
%For example, using this representation to describe a sentiment classification
%model might result in the following assignments:
%
%\begin{itemize}
%  \item $m$: a log-linear model
%  \item $\theta$: weights $\phi_1 \dots \phi_n$
%  \item $x$: a sentence of text
%  \item $\Phi$: a collection of features:
%    \begin{itemize}
%      \item $\phi_1(x)$: does the sentence contain a smiley face
%      \item $\phi_2(x)$: does the sentence contain a froney face
%      \item $\phi_n(x)$: does the sentence contain the word `happy'
%    \end{itemize}
%  \item $y$: whether the sentence has positive or negative sentiment
%\end{itemize}

%\textsc{Feature Cost} Each $\phi_i$ bears cost of computation to compute, with
%respect to the ``size'' of an input $x$, which we denote $s_i(x)$. For example,
%if $x$ is a sentence, a feature looking for a smiley face would have $s(x)$
%  which scales linearly with respect to the length of the sentence. If $x$ was
%  an array of integers, a feature which computed its median would have $s(x)$
%  which grew $n \lg n$  with respect to the size of the array $x$.
%
%\textsc{Performance} For any model $m$ and set of features $\Phi_i \subseteq
%\Phi$, we denote the performance of the model limited to just that set of
%features as $a(m, \Phi_i)$$
%


\section{Problem 1: Selecting features for a fixed problem size}

First we consider the case where the problem size ($|n|$) is fixed. I.e., at
runtime, the model will only be used on datasets of the same cardinality. If
this is the case, the naieve approach is then to calculate full set of possible
$F_i$ in $\mathcal F$ and evaluate the cost and accuracy offline, producing a
field of tradeoffs such as Figure~\ref{fig:tradeoff}.

\begin{figure}[h!]
\centering
\includegraphics[width=0.4\textwidth]{figures/cost-versus-errors.pdf}
\caption{Offline computation of all $F$.}
\label{fig:tradeoff}
\end{figure}

The subset of points which offer the best performance for a fixed range of
costs represents the \textbf{skyline} of our model. At runtime, for a given
budget, we picka  set of features $F_i$ from the skyline which is closest to
the budget without exceeding it.

The task here is how to efficiently compute this field of tradeoffs. Questions we have:

\begin{itemize}

 \item Do we assume that adding a feature necessarily improves performance?
 \item Do we assume that adding a feature necessarily improves cost?
 \item Do we assume intermediate data is not shared between feature functions? (i.e., mean and median could share state). Yes, for simplicity.
 \item 

\end{itemize}

\section{Problem 2: Dealing with varying problem sizes}

Recall that each features $f_i$ has a cost $c_i$ may be thought of as:

\[ c_i(x, n) = c_0 + c(x) + c_1 n + c_2 n^2 + \dots + c_k n^k \]

This means the tradeoffs between cost and performance change based on the size
of the dataset. But we assume the accuracy does not change.
Figure~\ref{fig:scale} shows a cartoon of of this.

\begin{figure}[h!]
\centering
\includegraphics[width=0.4\textwidth]{figures/scaling.pdf}
\caption{Points skew across the cost axis as $n$ changes.}
\label{fig:scale}
\end{figure}

Our second task is therefore to develop a data structure which allows us to
convert knowledge of the cost/performance tradeoffs of a universe of features
for a fixed $n$ such that we can make decisions for datasets of varying size.

It is not the case that the skyline will remain the same---albeit scaled to a
higher cost---for greater $n$ because constant and lower order factors may
dominate at low $n$ whereas higher order factors may dominate at high $n$.


\section{Problem 3: Relaxing the dataset size constraint}

In the previous problems, we have approached by the cost-optimization
problem by only considering the size of the inputs irrespective of
other features of the input.  However it is possible to achieve
much higher model accuracy by extending $select$ to consider other
attributes of the input.

For example, consider a credit rating agency that models the
probability of fraud given profiles of people.  It may be that the
optimal features for americans are job description and education
while those for europeans are home location and their twitter
profile.  Thus, during the training phase, we may consider partitioning
the learning problem by nationality and training different 

Let us extend $select$ as $select*$:

$$select*(\mathcal F, C, x, F_{s}) : <F_{next}, C'>$$

$select*$ accepts a new input: the set of features, $F_{s}$,
that have already been computed on x (e.g., $F_{s}(x)$ is
available).  Given this, $select*$ proposes a new set of features
to extract, $F_{next}$, and a new budget  $C' = C - cost(F_{next},
x)$.  The algorithm terminates when the budget $C$ has been exhausted.

Clearly, $F_{s}$ is a hugely large space, and learning a model for $select*$
may be too difficult.  Let us model this as a decision tree learning problem.

\begin{figure}[h!]
\centering
\includegraphics[width=0.25\textwidth]{figures/tree.pdf}
\caption{Graphical representation of the decision tree process for $select*$ problem.}  
\label{fig:tree}
\end{figure}



The decision tree (Figure~\ref{fig:tree}) consists of, and interleaves,
two types of nodes, $select_f$ (Triangle) and $select_c$ (Circle)
nodes, that make decisions based on features and budgets, respectively.
The input and outputs of both types of nodes is the tuple $<F_{s},
x, F_s(x), C>$.  Triangle nodes picks the next set of features,
$F_{next}$, extracts them, and updates the budget, given the features
that have been extracted so far (it does not consider $C$).  Its
output is thus $$<F_s \cup F_{next}, x, (F_s \cup F_{next})(x), C
- c_{next}(x)>$$  
Circle nodes pick the next triangle node based
on the value of $C$ without regard to the other values in the tuple
-- it is simply a routing node based on the remaining budget.  The
leaf nodes are always triangles that return the final set of features
to extract.

Concretely, consider the credit rating example earlier, and a new
user comes in.  If the $C < 10ms$, then $select*$ simply computes
and returns the feature $salary$.  However if $C > 10ms$, then the
triangle node extracts $F_2 = country$, which takes $6ms$.  The
country is USA so we take the left branch.  The circle considers
the remaining budget, $4ms$, and chooses the right branch, which
returns the optimal features $\{job, education\}$.  Thus the final
features are $\{country, job, education\}$.


\begin{figure}[h!]
\centering
\includegraphics[width=0.25\textwidth]{figures/naivetree.pdf}
\caption{Basic $select$ formulation under the decision tree model}
\label{fig:naivetree}
\end{figure}

Under this model, the basic $select$ operation in Problem 1 and 2
describes learning the three level decision tree depicted in
Figure~\ref{fig:naivetree}.  The root node always returns $F_{next}
= <size>$, the circle node picks a feature predictor based on the
budget, and the leaf triangle nodes return the optimal set of
features.


(Ted and I discussed another model where the $select$ problem could
be modeled as decision tree with nodes that only look at $<F_s =
\{size\}, C>$ while the $select*$ problem is modeled with nodes
that can look at $<F_s, x, C>$.  Unfortunately, I don't completely
remember.)

